Pegas: Perceptually Guided Heuristics for Accelerating Diffusion-based Video Streaming

Autoregressive video diffusion models enable streaming video generation but face substantial computational and memory costs that limit their efficiency and output resolution. Existing approaches commonly allocate resources uniformly across the visual field, overlooking the spatially varying sensitivity of human perception. We present Pegas, a perceptually guided heuristic for accelerating diffusion-based video streaming that allocates computation and memory throughout a frozen streaming video generator based on the viewer's gaze. Pegas integrates three key components: (1) gaze-guided generation that focuses late denoising steps near the gaze and caches past tokens according to perceptual importance; (2) foveated super-resolution that selectively refines gaze-centered regions while preserving global context through full-frame attention; (3) foveated decoding that reduces peripheral reconstruction costs through spatially adaptive resolution. To accommodate continuously changing gaze during streaming generation, we further introduce incremental super-resolution that dynamically updates refinement regions using the latest gaze measurements. Evaluated on an Ultra Flash backbone across 158 prompts with simulated human eye movements, Pegas achieves a 1.85x speed-up on one L40S and reduces mean peak memory from 32.8 to 21.7 GB at 1K. In a separate user study under central fixation, viewers rated Balanced level with Ultra Flash (+0.03 JOD) in overall quality and well above a uniform baseline at the same throughput.

==> figures/tex/speedVsJOD.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/pdf/speed_jod.pdf}
  \caption{\textbf{Speed against perceived quality.}
  Perceived quality in JOD relative to Ultra Flash from the user study (interim, 8 participants, 640 trials, central fixation), with 95\% bootstrap intervals over observers, against the speed-up over Ultra Flash on one L40S at 1K (\cref{tab:main}, TAEHV decoder).
  Marker area is proportional to mean peak VRAM. Filtered Ultra Flash runs at the speed of Ultra Flash and is drawn slightly to its left.
  \textit{Balanced} is $1.77\times$ faster than Ultra Flash at $-0.04$ JOD [$-0.48$, $0.38$], while spending the same compute uniformly loses $2.27$ JOD.
  The gaze-crop MUSIQ view and the per-condition JOD are in \cref{fig:speed-quality,fig:user-study} of the supplement.}
  \label{fig:speed-jod}
\end{figure}


==> sec/TODO.tex <==
TEAM TO-DO (not compiled into the paper). Rewritten Mon Nov 16, ~19:30 ET, at Henry's request. Line numbers refer to
the commit that adds this version (paper main eeab0e9 plus the KV figure in the supplement) and will drift.
Status:  [OPEN]  [IN PROGRESS]  [DECIDE] (needs Henry/Bingxuan)  [DONE]

No paper runs are in flight. The A6000 is idle, and Torch finished the last stage-ablation shards on 11-16 at
03:20 ET.
Tables 1-4 (tab:main, tab:others, tab:gpus, tab:stages) are frozen. Any change goes to Bingxuan first.

=====================================================================================================================
1. MAIN PAPER: NOT WRITTEN YET
=====================================================================================================================
[IN PROGRESS] (Henry) User study.
         - Written (A6000 hub, 11-16, r5 numbers from 1275c2f):
           - sec:user_study has the protocol, pwcmp scaling, intervals, Holm tests and exclusions.
           - "Quantitative results" has the JODs with intervals and p.
           - The supplement has its own "User study" section (sec:supp-study-all), with protocol, scaling and tests,
             and outlier screening with all 11 participants.
         - Open: the consent/IRB statement (\todo at the end of sec:user_study).
         - Done: pwcmp's Kolmogorov-Smirnov check (sec:supp-study-stats), run by the user-study session on r5.
           - Balanced, Fast and filtered Ultra Flash pass. Latent Upsampling and Uniform fail, at the scale's edge.
         - Done: the protocol facts were checked against the study config and clips (fixation cross, timing, question).
         - Done (Henry, 11-16): the IRB, consent and vision statement is in sec:user_study. The chin rest and the
           fixed distance are in the main text and in sec:supp-study-protocol. Participants were naive.
         - Done: the 20 prompts are a subset of the 158, picked by the Laplacian sharpness ranking (research-log
           5fbf3ba). sec:supp-study-protocol gives the ranking, the indices and the regeneration with center gaze.
         - Do not claim that Fast beats Latent Upsampling. It holds only with the two exclusions.

=====================================================================================================================
2. MAIN PAPER: DECISIONS
=====================================================================================================================
[DECIDE] KV budget wording, sec/3_method.tex L66: "spends it on the places the viewer has looked at".
         - At 25%, B = 8,190 tokens. That includes the sink frame and the newest four latent frames, which are kept
           in full (7,800 tokens), so only about 390 tokens are left for the gaze-scored history.
         - Either say that the budget includes the frames kept in full, or soften the claim. sec:supp-kv-impl should
           give the numbers.
         - This is the likely reason gaze KV ties the sliding window on gaze-crop MUSIQ.
[DECIDE] (Henry) A sentence on foveated FlashVSR in the main text?
         - It is currently only in the supplement (sec:supp-flashvsr).

=====================================================================================================================
3. MAIN PAPER: POLISH AND TRIM
=====================================================================================================================
[OPEN]   Shorten everything (all).
         - Candidates: the sec 4 setup and ablation paragraphs, and the user-study paragraph once it is written.
[OPEN]   sec/1_intro.tex L36: drop "preliminary", since the study is final. This is for the intro's owner.
[OPEN]   sec/0_abstract.tex L6 says "21.8 GB", but tab:main has 21.7 GB for both Balanced and Fast.
         - The intro's 34% holds either way.
[OPEN]   sec/3_method.tex L58: \TODO{fix this extra words that take up the line}. Trim the paragraph's last line.
[OPEN]   Simulated gaze (SQZ's comment, since removed from the intro): justify it in the main text.
         - The supplement has the recorded GazeCom gaze ("Recorded human gaze", 58% of frames inside the SR region)
           and the closed-loop test.
         - Neither sec:exp-gaze nor Limitations points to them.
[OPEN]   Refine the figures (all).
[OPEN]   (Henry) Citations: the final pass by hand, started Sat 14. Status unknown.
[OPEN]   (Colin) Go over the experiments. Assigned Sat 14; status unknown.
[OPEN]   Before submission:
         - Hide or remove every \TODO and \todo. preamble.tex L14-15 has the switches.
         - Delete the unused \pend and \pilot definitions (sec/4_experiments.tex L7-9).
         - Delete figures/tex/speedVsJOD.tex, which nothing \inputs.

=====================================================================================================================
4. TYPOS (proofread Mon Nov 16 against ae74e4f; every item was checked in the source). Fix it, then delete the line.
=====================================================================================================================
sec/0_abstract.tex L2: "a perceptually guided heuristics" -> "a set of perceptually guided heuristics".
sec/1_intro.tex L6: "highest at the foveal vision" -> "highest in foveal vision".
sec/3_method.tex L133: "\textit{Fast} enough for saccadic suppression" -> "fast enough ..." (the adjective, not the
  configuration).
sec/3_method.tex L154: "latest gaze sample~\cref{sec:exp-gaze}." -> "latest gaze sample (\cref{sec:exp-gaze}).".
sec/4_experiments.tex L55: "an \textit{Latent Upsampling}" -> "a \textit{Latent Upsampling}".
sec/4_experiments.tex L72 and L84: these sentences start with \cref{tab:main} and \cref{tab:others}, which print
  "Tab. 1". Use \Cref, as the rest of the paper does at the start of a sentence.
sec/5_limitations.tex L18: "framerates" -> "frame rates".
sec/5_limitations.tex L22: "26.91 for Fast" -> "26.91 for \textit{Fast}".
sec/X_suppl.tex L39: \paragraph{Stage timings with the tiny decoder.} has no text. Add one sentence that cites
  tab:tiny-stage-time.
sec/X_suppl.tex L124 and L164: "centre" -> "center". The rest of the paper uses American spelling.
sec/X_suppl.tex L126: "gaze-crop DINO similarity" -> "gaze-crop DINOv2 similarity", as on L132.
sec/X_suppl.tex L129, L140, L181 and L182: \ours{} prints a bold "Ours" in running text. Use \method{} (Pegas).
sec/X_suppl.tex L141: "from -1.25 to -1.10" -> "from $-1.25$ to $-1.10$" (minus signs, not hyphens).
sec/X_suppl_experiments.tex L20: "& -0.03 & -0.03" -> "& $-0.03$ & $-0.03$".
tables/ablation1.tex L26: "Ultra Flash output at gaze" -> "at the gaze". tab:stages is frozen, so Bingxuan makes this
  change.
tables/main_results.tex L34: the caption says bold marks the column bests among accelerated configurations.
  - The Foveated SR row (1.43x) beats the bold Balanced values in KID (3.07 vs 4.38), AQ and HPS, and it ties Latent
    Upsampling's bold Avg. (74.98).
  - Either limit the caption to the configuration and alternative rows, or change the bolding.
  - tab:main is frozen, so Bingxuan makes this change.

=====================================================================================================================
5. SUPPLEMENT: STUBS AND CAPTIONS (sec/X_suppl.tex unless noted)
=====================================================================================================================
[OPEN]   L96, "Shorter SR calls": the 1.5 s call split into three 0.5 s calls, and the call-length sweep.
[OPEN]   L101, "Recent-gaze heatmap": the oracle ceiling and the centre-prior analysis.
[OPEN]   L213, sec:supp-saliency: the saliency head's architecture (0.48M parameters), its training against UNISAL,
         and its runtime (0.7 ms per frame).
[OPEN]   L231, sec:supp-kv-impl (fig:kv-anatomy is already there):
         - the fused log-bias kernel, the side-stream compaction and the budget allocation;
         - the pooled-entry ablation;
         - the budget numbers from section 2.
[OPEN]   L237, sec:supp-washout: the RoPE wash-out figure and the position-renumbering fix.
[OPEN]   L240, "Region-adaptive denoising": the drift analysis, the 2-of-3 alternation, the 10 deg radius and the
         cut timestep.
         - Check the "900" in the TODO against sec:method-ra, which skips t = 833 and 625 after step k* = 2.
[OPEN]   L243, "Foveated SR and decoding": the SR cache detail, the crop-vs-ours seams and the decoding settings.
[OPEN]   L253, fig:supp-timestrip: still the placeholder from placeholders.py.
         - Henry's plan: columns at t = 0, 2.5, 5, ... s, and one row per method, each followed by a row of its gaze
           and periphery crops.
         - The clips still need to be rendered.
[OPEN]   L259, "Profiling": per-stage wall clock of Ultra Flash and Ours.
         - The FPS accounting is already in "Throughput with overlapping stages" (L58), so that part can leave this
           TODO.
[DECIDE] L295, "Extended baselines": KV at 50%, head-level pruning, FP8, and the full FlashVSR comparison. Keep or
         cut each.
[OPEN]   figures/tex/speedVsQuality.tex L7: \TODO{Improve and finalize the figure and caption.}
[DECIDE] FOCAS (Bingxuan, focas_check_v3) and the 5 deg Foveated Diffusion port (Henry) were planned for the
         supplement but are not in it. Add or drop.
[DECIDE] Filter anchor: s = 0.815 was calibrated on the v3 release at 1K, not on TAEHV ("P1 anchor re-filter" in
         Bingxuan's plan).
         - Rerun it, or state this in the calibration paragraph (X_suppl_experiments.tex L63).

=====================================================================================================================
6. DONE (details are in this file's git history, on agent-comms and in research-log)
=====================================================================================================================
Tables
  - tab:main, tab:others, tab:gpus (4090, A6000, L40S and H100, 1K and 2K) and tab:stages (158 prompts) are final
    and frozen.
  - Table 2 as differences to Ultra Flash was not adopted; the values are in this file's history.
Figures
  - Pipeline (fig:pipeline, figures/pdf/pipeline.pdf) is final (Henry, 11-16).
  - KV memory (fig:kv-anatomy) is in the supplement, sec:supp-kv-impl (Henry, 11-16).
  - Teaser: P86 frames, with panel (c) showing the user study against the speed-up.
  - Qualitative: bird, rose and cow, with gaze and periphery crops.
  - fig:user-study and speed vs quality (158-prompt intervals; its caption TODO is above).
  - Region share.
User study
  - Collection is closed. The final results (r5, 1275c2f) are 9 analysed of 11 tested, 720 trials.
  - The all-11 table is in sec:supp-study-all, and pwcmp is cited.
Method
  - Region-adaptive denoising, KV memory, the commit horizon, gaze prediction, foveated SR and foveated decoding are
    all written.
  - The intro's contributions cover region-adaptive denoising and the KV cache in one bullet (Bingxuan, 0586a76).
Supplement sections written
  - Evaluation and timing: common display size, timing boundaries, stage timings, the two-GPU schedule.
  - Gaze: placement, size and latency; the gaze oracle; the closed loop; the recorded GazeCom gaze.
  - Other: foveated FlashVSR, whole-frame and acuity KID, filter sensitivity, the VBench breakdown, content fidelity,
    component removal, and the Wan2.1 speed estimate.
Other
  - The filter is csf10x0.815.
  - Limitations and Conclusion are their own sections.

=====================================================================================================================
7. FUTURE WORK / IF TIME
=====================================================================================================================
[OPEN]   H200: why are its results poor? H200 is not in tab:gpus.


For future revisions:
argue better that streaming is non trivial, since foveated diffusion requires knowing the gaze scanpath in advanced
